Evaluation and Improvement of Interpretability for Self-Explainable Part-Prototype Networks

Part-prototype networks (e.g., ProtoPNet, ProtoTree, and ProtoPool) have attracted broad research interest for their intrinsic interpretability and comparable accuracy to non-interpretable counterparts. However, recent works find that the interpretability from prototypes is fragile, due to the semantic gap between the similarities in the feature space and that in the input space. In this work, we strive to address this challenge by making the first attempt to quantitatively and objectively evaluate the interpretability of the part-prototype networks. Specifically, we propose two evaluation metrics, termed as consistency score and stability score, to evaluate the explanation consistency across images and the explanation robustness against perturbations, respectively, both of which are essential for explanations taken into practice. Furthermore, we propose an elaborated part-prototype network with a shallow-deep feature alignment (SDFA) module and a score aggregation (SA) module to improve the interpretability of prototypes. We conduct systematical evaluation experiments and provide substantial discussions to uncover the interpretability of existing part-prototype networks. Experiments on three benchmarks across nine architectures demonstrate that our model achieves significantly superior performance to the state of the art, in both the accuracy and interpretability. Our code is available at https://github.com/hqhQAQ/EvalProtoPNet.

==> figs/reasoning_vis.tex <==
\begin{figure}[ht]
\centering
    \includegraphics[width=\linewidth]{imgs/reasoning.pdf}
\caption{Reasoning process for a Painted Bunting.}
% The prototypes accurately match the test bird’s leg, head and wing with that in the training images, providing evidences for the bird classification.
\label{fig:reasoning_process}
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/ablation_consis_coe.tex <==
\begin{table*}
\small
\renewcommand\arraystretch{1.5}
\centering
\setlength{\tabcolsep}{1.2mm}{
\begin{tabular}{c|*3{c}|*3{c}|*3{c}|*3{c}|*3{c}}
  \toprule
\multirow{2}*{\normalsize \textbf{Backbone}} & \multicolumn{3}{c|}{\normalsize \textbf{0.30}}  & \multicolumn{3}{c|}{\normalsize \textbf{0.40}} & \multicolumn{3}{c|}{\normalsize \textbf{0.50${}^{\dagger}$}} & \multicolumn{3}{c|}{\normalsize \textbf{0.60}} & \multicolumn{3}{c}{\normalsize \textbf{0.70}} \\

% \hhline{*{1}{|~}*{9}{|-}|~|}
\cline{2-16}

& \textbf{\normalsize Con.} & \textbf{\normalsize Sta.} & \textbf{\normalsize Acc.} & \textbf{\normalsize Con.} & \textbf{\normalsize Sta.} & \textbf{\normalsize Acc.} & \textbf{\normalsize Con.} & \textbf{Sta.} & \textbf{\normalsize Acc.} & \textbf{\normalsize Con.} & \textbf{\normalsize Sta.} & \textbf{\normalsize Acc.} & \textbf{\normalsize Con.} & \textbf{\normalsize Sta.} & \textbf{\normalsize Acc.} \\

\midrule

{\normalsize ResNet34} & 69.5 & 70.6 & 83.7 & 70.4 & 71.2 & 83.7 & 70.6 & 72.1 & 84.0 & 71.5 & 72.4 & 83.8 & 71.8 & 72.4 & 83.6 \\
{\normalsize VGG19} & 53.5 & 62.4 & 82.6 & 56.6 & 62.5 & 82.8 & 56.5 & 63.5 & 82.5 & 58.4 & 63.9 & 82.5 & 58.9 & 64.8 & 82.2 \\
{\normalsize Dense121} & 67.1 & 65.4 & 85.4 & 67.9 & 66.5 & 85.2 & 68.1 & 67.6 & 85.4 & 69.7 & 68.0 & 85.2 & 70.5 & 68.6 & 84.8 \\

\bottomrule
\end{tabular}}
%   }
\caption{Ablation experiments of the coefficient $\lambda_{\mathrm{align}}$ of the alignment loss $\mathcal{L}_{\mathrm{align}}$ on \emph{CUB-200-2011}. $\dagger$ denotes the parameter we choose in the main experiments. The results indicate that the increase of $\lambda_{\mathrm{align}}$ improves the consistency score and stability score of our model, but a too high $\lambda_{\mathrm{align}}$ may affect the learning of classification loss and thus hurts the accuracy.}
\label{tab:ablation_consis_coe}

\end{table*}

==> tables/ablation_consis_thresh.tex <==
\begin{table*}
\small
\renewcommand\arraystretch{1.5}
\centering
\setlength{\tabcolsep}{1.2mm}{
\begin{tabular}{c|*3{c}|*3{c}|*3{c}|*3{c}|*3{c}}
  \toprule
\multirow{2}*{\normalsize \textbf{Backbone}} & \multicolumn{3}{c|}{\normalsize \textbf{0.05}}  & \multicolumn{3}{c|}{\normalsize \textbf{0.10${}^{\dagger}$}} & \multicolumn{3}{c|}{\normalsize \textbf{0.15}} & \multicolumn{3}{c|}{\normalsize \textbf{0.20}} & \multicolumn{3}{c}{\normalsize \textbf{0.25}} \\

% \hhline{*{1}{|~}*{9}{|-}|~|}
\cline{2-16}

& \textbf{\normalsize Con.} & \textbf{\normalsize Sta.} & \textbf{\normalsize Acc.} & \textbf{\normalsize Con.} & \textbf{\normalsize Sta.} & \textbf{\normalsize Acc.} & \textbf{\normalsize Con.} & \textbf{Sta.} & \textbf{\normalsize Acc.} & \textbf{\normalsize Con.} & \textbf{\normalsize Sta.} & \textbf{\normalsize Acc.} & \textbf{\normalsize Con.} & \textbf{\normalsize Sta.} & \textbf{\normalsize Acc.} \\

\midrule

{\normalsize ResNet34} & 72.4 & 72.3 & 83.5 & 70.6 & 72.1 & 84.0 & 69.9 & 71.2 & 83.9 & 68.8 & 70.6 & 84.2 & 69.3 & 69.5 & 83.8 \\
{\normalsize VGG19} & 58.6 & 64.2 & 82.1 & 56.5 & 63.5 & 82.5 & 56.6 & 62.7 & 82.5 & 55.9 & 62.8 & 82.8 & 55.5 & 62.0 & 82.7 \\
{\normalsize Dense121} & 71.2 & 67.8 & 84.8 & 68.1 & 67.6 & 85.4 & 67.7 & 66.9 & 85.4 & 66.5 & 65.2 & 85.2 & 67.4 & 64.3 & 85.1 \\

\bottomrule
\end{tabular}}
%   }
\caption{Ablation experiments of the thresh $\gamma$ of the alignment loss $\mathcal{L}_{\mathrm{align}}$ on \emph{CUB-200-2011}. $\dagger$ denotes the parameter we choose in the main experiments. The results indicate that the decrease of $\gamma$ improves the consistency score and stability score of our model. But similar to $\lambda_{\mathrm{align}}$, a too small $\gamma$ hurts the accuracy.}
\label{tab:ablation_consis_thresh}

\end{table*}

==> tables/benchmark_car.tex <==
\begin{table*}
\small
\renewcommand\arraystretch{1.15}
\centering
\setlength{\tabcolsep}{1.2mm}{
\begin{tabular}{c|c|c|c|c|c|c}
  \toprule
{\normalsize \textbf{Method}} & {\normalsize \textbf{ResNet34}}  & {\normalsize \textbf{ResNet152}} & {\normalsize \textbf{VGG16}} & {\normalsize \textbf{VGG19}} & {\normalsize \textbf{Dense121}} & {\normalsize \textbf{Dense161}} \\

% \hhline{*{1}{|~}*{9}{|-}|~|}

% & \textbf{\normalsize Con.} & \textbf{\normalsize Sta.} & \textbf{\normalsize Acc.} & \textbf{\normalsize Con.} & \textbf{\normalsize Sta.} & \textbf{\normalsize Acc.} & \textbf{\normalsize Con.} & \textbf{Sta.} & \textbf{\normalsize Acc.} & \textbf{\normalsize Con.} & \textbf{\normalsize Sta.} & \textbf{\normalsize Acc.} & \textbf{\normalsize Con.} & \textbf{\normalsize Sta.} & \textbf{\normalsize Acc.} \\

\midrule

{\normalsize ProtoTree}~\cite{abla_meike2021ProtoTree} & 86.6 & N/A & N/A & N/A & N/A & N/A \\
{\normalsize ProtoPNet}~\cite{abla_chen19ProtoPNet} & 88.8 & 88.5 & 88.3 & 89.4 & 87.7 & 89.5 \\
{\normalsize ProtoPool}~\cite{abla_Ryma2021Assignment} & 89.3 & N/A & N/A & N/A & N/A & N/A \\
{\normalsize TesNet}~\cite{abla_jiaqi2021TesNet} & 90.9 & 92.0 & 90.3 & 90.6 & 91.9 & 92.6 \\

\hline

{\normalsize Ours + SA + SDFA} & \textbf{92.0} & \textbf{92.8} & \textbf{90.8} & \textbf{91.0} & \textbf{92.4} & \textbf{92.9} \\

\bottomrule
\end{tabular}}
%   }
\caption{The accuracy of part-prototype networks on \emph{Stanford Cars}. The results are over six convolutional backbones pre-trained on ImageNet.}
% Our results are averaged over 4 runs with different seeds. Bold font denotes the best result.
\label{tab:car_benchmark}

\end{table*}

==> tables/benchmark_cub_vit.tex <==
\begin{table*}
\small
\renewcommand\arraystretch{1.15}
\centering
\setlength{\tabcolsep}{1.4mm}{
\begin{tabular}{c|*3{c}|*3{c}|*3{c}}
  \toprule
\multirow{2}*{\small \textbf{Method}} & \multicolumn{3}{c|}{\small \textbf{DeiT-Ti}}  & \multicolumn{3}{c|}{\small \textbf{DeiT-S}} & \multicolumn{3}{c}{\small \textbf{DeiT-B}} \\

% \hhline{*{1}{|~}*{9}{|-}|~|}
\cline{2-10}

& \textbf{\small Con.} & \textbf{\small Sta.} & \textbf{\small Acc.} & \textbf{\small Con.} & \textbf{\small Sta.} & \textbf{\small Acc.} & \textbf{\small Con.} & \textbf{Sta.} & \textbf{\small Acc.} \\

\midrule

{\small Baseline} & N/A & N/A & 81.2 & N/A & N/A & 82.2 & N/A & N/A & 82.5 \\
{\small ProtoPNet~\cite{abla_chen19ProtoPNet}} & 27.3 & 59.0 & 77.2 & 12.3 & 57.5 & 78.1 & 16.9 & 56.6 & 76.0 \\
{\small TesNet~\cite{abla_jiaqi2021TesNet}} & 38.4 & 61.4 & 81.2 & 29.0 & 63.1 & 80.4 & 36.2 & 62.4 & 82.9 \\
\hline

{\small Ours + SA + SDFA} & \textbf{48.8} & \textbf{65.7} & \textbf{84.3} & \textbf{58.3} & \textbf{67.9} & \textbf{84.6} & \textbf{51.7} & \textbf{70.4} & \textbf{85.0} \\

\bottomrule
\end{tabular}}
%   }
\caption{Evaluation results of interpretability and accuracy of part-prototype networks on \emph{CUB-200-2011}. The results are over three ViT backbones pre-trained on ImageNet. Con., Sta. and Acc. denote consistency score, stability score and accuracy, respectively. Bold font denotes the best result.}
\label{tab:cub_vit_benchmark}

\end{table*}

==> tables/benchmark_params.tex <==
\begin{table*}
\small
\renewcommand\arraystretch{1.15}
\centering
\setlength{\tabcolsep}{1.2mm}{
\begin{tabular}{c|c|c|c|c|c}
  \toprule
{\normalsize \textbf{Method}} & {\normalsize \textbf{ResNet34}}  & {\normalsize \textbf{ResNet152}} & {\normalsize \textbf{VGG19}} & {\normalsize \textbf{Dense121}} & {\normalsize \textbf{Dense161}} \\

% \hhline{*{1}{|~}*{9}{|-}|~|}

% & \textbf{\normalsize Con.} & \textbf{\normalsize Sta.} & \textbf{\normalsize Acc.} & \textbf{\normalsize Con.} & \textbf{\normalsize Sta.} & \textbf{\normalsize Acc.} & \textbf{\normalsize Con.} & \textbf{Sta.} & \textbf{\normalsize Acc.} & \textbf{\normalsize Con.} & \textbf{\normalsize Sta.} & \textbf{\normalsize Acc.} & \textbf{\normalsize Con.} & \textbf{\normalsize Sta.} & \textbf{\normalsize Acc.} \\

\midrule

{\normalsize Baseline} & \textbf{21.39M} & 58.55M & \textbf{20.17M} & 7.16M & 26.91M \\
{\normalsize ProtoTree}~\cite{abla_meike2021ProtoTree} & 21.55M & 58.80M & 20.29M & 7.35M & 27.17M  \\
{\normalsize ProtoPNet}~\cite{abla_chen19ProtoPNet} & 22.02M & 59.08M & 20.76M & 7.76M & 27.43M  \\
{\normalsize ProtoPool}~\cite{abla_Ryma2021Assignment} & 22.27M & 59.53M & 21.01M & 8.07M & 27.90M  \\
{\normalsize Deformable}~\cite{abla_Jon2022Deform} & 26.84M & 79.13M & 25.58M & 17.65M & 49.07M \\
{\normalsize TesNet}~\cite{abla_jiaqi2021TesNet} & 21.85M & 58.80M & 20.59M & 7.55M & 27.14M \\

\hline

{\normalsize Ours + SA + SDFA} & 21.45M & \textbf{58.40M} & 20.19M & \textbf{7.15M} & \textbf{26.74M} \\

\bottomrule
\end{tabular}}
%   }
\caption{The number of parameters in different part-prototype networks (Measured on \emph{CUB-200-2011}). Bond font denotes the minimum number of parameters.}
% Our results are averaged over 4 runs with different seeds. Bold font denotes the best result.
\label{tab:params_benchmark}

\end{table*}

==> tables/benchmark_partimgnet.tex <==
\begin{table*}
\small
\renewcommand\arraystretch{1.15}
\centering
\setlength{\tabcolsep}{1.4mm}{
\begin{tabular}{c|*3{c}|*3{c}|*3{c}|*3{c}|*3{c}}
  \toprule
\multirow{2}*{\small \textbf{Method}} & \multicolumn{3}{c|}{\small \textbf{ResNet34}}  & \multicolumn{3}{c|}{\small \textbf{ResNet152}} & \multicolumn{3}{c|}{\small \textbf{VGG19}} & \multicolumn{3}{c|}{\small \textbf{Dense121}} & \multicolumn{3}{c}{\small \textbf{Dense161}} \\

% \hhline{*{1}{|~}*{9}{|-}|~|}
\cline{2-16}

& \textbf{\small Con.} & \textbf{\small Sta.} & \textbf{\small Acc.} & \textbf{\small Con.} & \textbf{\small Sta.} & \textbf{\small Acc.} & \textbf{\small Con.} & \textbf{Sta.} & \textbf{\small Acc.} & \textbf{\small Con.} & \textbf{\small Sta.} & \textbf{\small Acc.} & \textbf{\small Con.} & \textbf{\small Sta.} & \textbf{\small Acc.} \\

\midrule

{\small ProtoPNet~\cite{abla_chen19ProtoPNet}} & 15.6 & 70.3 & 79.3 & 27.3 & 72.7 & 82.4 & 15.7 & 69.7 & 77.3 & 11.6 & 69.1 & 80.6 & 10.6 & 70.1 & 83.4 \\
{\small TesNet~\cite{abla_jiaqi2021TesNet}} & 42.8 & 82.1 & 83.5 & 36.7 & 77.0 & 87.1 & 23.9 & 71.3 & 81.2 & 47.3 & 77.8 & 83.9 & 48.1 & 80.8 & 86.3 \\
\hline

{\small Ours + SA + SDFA} & \textbf{47.5} & \textbf{85.6} & \textbf{85.2} & \textbf{53.9} & \textbf{84.0} & \textbf{88.9} & \textbf{34.5} & \textbf{73.8} & \textbf{82.6} & \textbf{49.5} & \textbf{83.4} & \textbf{85.7} & \textbf{55.3} & \textbf{85.2} & \textbf{88.8} \\

\bottomrule
\end{tabular}}
%   }
\caption{The comprehensive evaluation of interpretability and accuracy of part-prototype networks on \emph{PartImageNet}. The results are over five convolutional backbones pre-trained on ImageNet. Con., Sta. and Acc. denote consistency score, stability score and accuracy, respectively. Bold font denotes the best result.}
\label{tab:partimgnet_benchmark}

\end{table*}

==> tables/notations.tex <==
\begin{table*}
\renewcommand\arraystretch{1.15}
\small
\centering
\setlength{\tabcolsep}{0.5mm}{
\begin{tabular}{c|l|c|l}
  \toprule
\textbf{Symbol} & \makecell[r]{\textbf{Description}} & \textbf{Symbol} & \makecell[r]{\textbf{Description}} \\

\midrule

$x$ & Input image & $c(j)$ & The allocated category of prototype $\boldsymbol{\mathrm{p}}_j$ \\
$f$ & Convolutional network of ProtoPNet & $a^{\boldsymbol{\mathrm{p}}_j}$ & Averaged corresponding object parts of $\boldsymbol{\mathrm{p}}_j$, $a^{\boldsymbol{\mathrm{p}}_j} \in \mathbb{R}^{C}$ \\
$g_{\boldsymbol{\mathrm{p}}}$ & Prototype layer of ProtoPNet & $\mu$ & Threshold for determination of consistency of prototypes \\
$h$ & Fully-connected layer of ProtoPNet & $S_{\mathrm{con}}$ & Consistency score of ProtoPNet \\
$K$ & Number of categories in the dataset & $\xi$ & Noise for determination of stability of prototypes \\
$M$ & Number of prototypes in $g_{\boldsymbol{\mathrm{p}}}$ & $S_{\mathrm{sta}}$ & Stability score of ProtoPNet \\
$N$ & Number of prototypes allocated to each category & $t(z)$ & Spatial similarity structure of $z$, $t(z) \in \mathbb{R}^{HW \times HW}$ \\
$D$ & Dimension of the prototype & $H_s, W_s, D_s$ & Height, width and dimension of a shallow feature map \\
$\boldsymbol{\mathrm{P}}$ & The set of $M$ prototypes in $g_{\boldsymbol{\mathrm{p}}}$ & $H_d, W_d, D_d$ & Height, width and dimension of a deep feature map \\
$\boldsymbol{\mathrm{p}}_j$ & The $j$-th prototype in $\boldsymbol{\mathrm{P}}$, $\boldsymbol{\mathrm{p}}_j \in \mathbb{R}^{1 \times 1 \times D}$ & $z_s$ & A shallow feature map, $z_s \in \mathbb{R}^{H_s W_s \times D_s}$ \\
$D$ & Dimension of the prototype & $z_d$ & A deep feature map, $z_d \in \mathbb{R}^{H_d W_d \times D_d}$ \\
$H$, $W$ & Height and width of the feature map & $\mathcal{L}_{\mathrm{align}}$ & The shallow-deep feature alignment loss \\
$z$ & The feature map extracted by $f$, $z \in \mathbb{R}^{H \times W \times D}$ & $\mathrm{logit}_k$ & Classification score of category $k$ \\
$\tilde{z}$ & A unit of $z$, $\tilde{z} \in \mathbb{R}^{1 \times 1 \times D}$ & $\gamma$ & Threshold for $\mathcal{L}_{\mathrm{align}}$ \\
$v^{\boldsymbol{\mathrm{p}}_j}(x)$ & The activation map of $\boldsymbol{\mathrm{p}}_j$ on $z$, $v^{\boldsymbol{\mathrm{p}}_j}(x) \in \mathbb{R}^{H \times W}$ & $w^{\mathrm{SA}}$ & Weight of SA module, $w^{\mathrm{SA}} \in \mathbb{R}^{M}$ \\
$g^{\boldsymbol{\mathrm{p}}_j}(x)$ & The activation value of $\boldsymbol{\mathrm{p}}_j$ on $z$ & $\tilde{w}^{\mathrm{SA}}$ & Normalization of $w^{\mathrm{SA}}$ \\
$\mathrm{Sim}(\cdot, \cdot)$ & Similarity score between two vectors & $\mathcal{L}_{\mathrm{total}}$ & The total loss \\
$r^{\boldsymbol{\mathrm{p}}_j}(x)$ & The corresponding region of $\boldsymbol{\mathrm{p}}_j$ on $x$ & $\boldsymbol{\mathrm{P}}^k$ & Concatenation of prototypes from category $k$, $\boldsymbol{\mathrm{P}}^k \in \mathbb{R}^{N \times D}$ \\
$H_b, W_b$ & Height and width of the corresponding region & $\mathbb{I}_{N}$ & The $N \times N$ identity matrix \\
$C$ & Number of categories of object parts in the dataset & $\mathcal{L}_{\mathrm{ortho}}$ & The orthogonality loss \\
$o^{\boldsymbol{\mathrm{p}}_j}(x)$ & Corresponding object parts of $\boldsymbol{\mathrm{p}}_j$ on $x$, $o^{\boldsymbol{\mathrm{p}}_j}(x) \in \mathbb{R}^{C}$ & $\mathcal{L}_{\mathrm{clst}}$ & The cluster loss \\
$u(x)$ & Visible object parts in $x$, $u(x) \in \mathbb{R}^{C}$ & $\lambda_{\mathrm{align}}$ & Coefficient of $\mathcal{L}_{\mathrm{align}}$ \\
$\mathcal{I}_{k}$ & Test images belonging to category $k$ & $\mathcal{L}_{\mathrm{ce}}$ & The cross entropy loss \\
$\oplus$ & Concatenation of two vectors & $\mathcal{L}_{\mathrm{sep}}$ & The separation loss \\

\bottomrule
\end{tabular}}
%   }
\caption{Summary of notations used in the main body of this paper.}
\label{tab:notations}

\end{table*}

==> tables/revised_protopnet.tex <==
\begin{table}
\renewcommand\arraystretch{1.15}
\small
\centering
\setlength{\tabcolsep}{0.94mm}{
\begin{tabular}{c|c|c}
  \toprule
\textbf{Differences} & \textbf{Vanilla ProtoPNet} & \textbf{Revised Baseline} \\

\midrule

Cluster Loss & \Checkmark & \XSolidBrush \\
Separation Loss & \Checkmark & \XSolidBrush \\
$L_1$ Loss & \Checkmark & \XSolidBrush \\
Orthogonality Loss & \XSolidBrush & \Checkmark \\
Prototype Projection & \Checkmark & \XSolidBrush \\
Convex Optimization & \Checkmark & \XSolidBrush \\
Activation Function & $\mathrm{log}\Big( \frac{\| \tilde{z} - \boldsymbol{\mathrm{p}}_j \|^{2} + 1}{\| \tilde{z} - \boldsymbol{\mathrm{p}}_j \|^{2} + \epsilon} \Big)$ & $\langle \tilde{z}, \boldsymbol{\mathrm{p}}_j \rangle$ \\
Add-on Module & Double Layers & Single Layer \\
Decay Epochs & 5 & 2 \\
Decay Rate & 0.1 & 0.4 \\

\bottomrule
\end{tabular}}
%   }
\caption{Differences between our revised ProtoPNet and the vanilla ProtoPNet. \Checkmark denotes the operation is adopted and \XSolidBrush otherwise.}
\label{tab:revised_protopnet}

\end{table}

==> tables/stability_variants.tex <==
\begin{table}
\setlength{\abovecaptionskip}{0.1cm}
\footnotesize
\centering
\renewcommand\arraystretch{1.15}
\setlength{\tabcolsep}{0.6mm}{
\begin{tabular}{c|c|c|c|c|c|c}
  \toprule
{\textbf{\small Method}} & {\textbf{ProtoTree}}  & {\textbf{ProtoPNet}} & \textbf{ProtoPool} & {\textbf{Deform.}} & {\textbf{TesNet}} & {\textbf{Ours}} \\
\midrule
\textbf{\small Original} & 21.6 & 53.8 & 57.6 & 57.0 & 65.4 & \textbf{72.1} \\
\textbf{\small IoU} & 18.2 & 35.1 & 38.5 & 41.4 & 56.7 & \textbf{70.4} \\
\textbf{\small PGD} & 16.4 & 26.2 & 39.9 & 36.5 & 53.1 & \textbf{60.8} \\
\bottomrule
\end{tabular}}
\caption{\textbf{Original:} The original stability score in the main paper. \textbf{IoU:} The stability score calculated with IoU. \textbf{PGD:} The stability score calculated using PGD attack for noise production. The results are from \emph{CUB-200-2011} 
on ResNet34 backbone.}
\label{tab:stability_iou_pgd}
\end{table}
